TSM: Temporal Shift Module for Efficient and Scalable Video Understanding on Edge Device

The explosive growth in video streaming requires video understanding at high accuracy and low computation cost. Conventional 2D CNNs are computationally cheap but cannot capture temporal relationships; 3D CNN-based methods can achieve good performance but are computationally intensive. In this paper, we propose a generic and effective Temporal Shift Module (TSM) that enjoys both high efficiency and high performance. The key idea of TSM is to shift part of the channels along the temporal dimension, thus facilitate information exchanged among neighboring frames. It can be inserted into 2D CNNs to achieve temporal modeling at zero computation and zero parameters. TSM offers several unique advantages. Firstly, TSM has high performance; it ranks the first on the Something-Something leaderboard upon submission. Secondly, TSM has high efficiency; it achieves a high frame rate of 74fps and 29fps for online video recognition on Jetson Nano and Galaxy Note8. Thirdly, TSM has higher scalability compared to 3D networks, enabling large-scale Kinetics training on 1,536 GPUs in 15 minutes. Lastly, TSM enables action concepts learning, which 2D networks cannot model; we visualize the category attention map and find that spatial-temporal action detector emerges during the training of classification tasks. The code is publicly available at https://github.com/mit-han-lab/temporal-shift-module.

==> figureText/fig_arrow_of_time.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figures/arrow_of_time.pdf}
\caption{
Something-Something dataset is temporal-related. Following different arrows of time gives different labels of the dataset.}
\label{fig:array_of_time}
% \vspace{-15pt}
\end{figure}

==> figureText/fig_overall.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{figures/overall.pdf}
\caption{The architecture of \netFull framework. The video is splitted into $N$ segments of equal size. One frame is sampled from each segment. We use 2D convolution to extract the spatial feature from each frame. The \method module is inserted afterwards to conduct temporal fusion at no cost.}
\label{fig:overall}
% \vspace{-15pt}
\end{figure*}

==> figureText/fig_tsm_module.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.31\textwidth}
	\includegraphics[width=\textwidth]{figures/shift_ori_pad.pdf}
	\caption{The original tensor without temporal fusion. $Row_i$ only contains the feature maps from $T_i$.}
	\label{fig:shift_ori}
\end{subfigure}
~~~~
\begin{subfigure}[b]{0.31\textwidth}
	\includegraphics[width=\textwidth]{figures/shift_zero_pad.pdf}
	\caption{Tensor with temporal shift (zero padding). $Row_i$ contains the feature maps from $T_{i-1}$, $T_{i}$ and $T_{i+1}$ (except boundary).}
	\label{fig:shift_zero}
\end{subfigure}
~~~~
\begin{subfigure}[b]{0.31\textwidth}
	\includegraphics[width=\textwidth]{figures/shift_circulant_pad.pdf}
	\caption{Tensor with temporal shift (circulant padding). $Row_i$ contains the feature maps from $T_{i-1}$, $T_{i}$ and $T_{i+1}$.}
	\label{fig:shift_circulant}
\end{subfigure}
\caption{Temporal shift module. For an activation tensor $A \in \mathbb{R}^{N\times T\times C\times H \times W}$, we display the $T$ and $C$ dimensions here. For a conventional 2D CNN, it operates on different frames independently (each frame is a row with the same color). While with our \method module,  adjacent three frames are mingled together (multiple colors per row). Temporal shift module has zero parameter overhead, zero computation overhead, yet effectively mixes the temporal information from adjacent frames. }
% \vspace{-10pt}
\label{fig:shift}
\end{figure*}

==> figureText/tab_compare_2d.tex <==
% \renewcommand \arraystretch{1}
% \begin{table}[t]
% %\setlength{\tabcolsep}{3pt}
% \caption{Our method consistently outperforms 2D counterparts on multiple datasets at zero extra cost. All the results are reported on the validation set using RGB modality and only 1 crop for efficiency. All the models use ResNet-50 backbone, with the same training protocol.}
% % \vspace{-6pt}
% \label{tab:compared_2d}
% \small
% \begin{center}
% \begin{tabular}{cccccc}
% \toprule
% \textbf{Dataset} & \textbf{\#Frame}& \textbf{Model} &  \textbf{Acc1} &  \textbf{Acc5} &  \textbf{$\Delta$ Acc1}  \\ 
% \toprule
% % Kinetics
% \multirow{4}{*}{Kinetics} & \multirow{2}{*}{8} & TSN & 68.8 & 88.3 & \multirow{2}{*}{+1.8}  \\ 
% % TRN_kinetics_RGB_resnet50_shift_shift8_blockres_avg_segment8_e45_tunek
%  &  & Ours & \textbf{70.6} & \textbf{89.5} \\ \cmidrule(l){2-6}
% & \multirow{2}{*}{16} & TSN & 69.4 & 88.7  & \multirow{2}{*}{+3.1} \\ 
% % TRN_kinetics_RGB_resnet50_shift_shift8_blockres_avg_segment16_e30_tunek
%  &  & Ours & \textbf{72.5} & \textbf{90.7} \\  \midrule
% % UCF-101
% % TRN_ucf101_RGB_resnet50_avg_segment8_e25_tunekk
% \multirow{4}{*}{UCF101} & \multirow{2}{*}{8} & TSN & 91.5 & 99.2 & \multirow{2}{*}{+2.5} \\ 
% % TRN_ucf101_RGB_resnet50_shift_shift8_blockres_avg_segment8_e25_tunekk
%  &  & Ours & \textbf{94.0} & \textbf{99.2} \\ \cmidrule(l){2-6}
% & \multirow{2}{*}{16} & TSN & 91.4 & 99.2& \multirow{2}{*}{+3.1}  \\ 
%  &  & Ours & \textbf{94.5} & \textbf{99.5} \\  \midrule
% % HMDB 
% \multirow{4}{*}{HMDB51} & \multirow{2}{*}{8} & TSN & 64.8 & 89.1 & \multirow{2}{*}{+5.5} \\ 
%  &  & Ours & \textbf{70.3} & \textbf{92.4} & \\ \cmidrule(l){2-6}
% & \multirow{2}{*}{16} & TSN & 65.2 & 89.5 & \multirow{2}{*}{+5.5} \\ 
%  &  & Ours & \textbf{70.7} & \textbf{91.8} \\   
% \midrule \midrule
% % Something V1 
% \multirow{4}{*}{\shortstack{Something\\V1}} & \multirow{2}{*}{8} & TSN & 19.7  & 46.6 & \multirow{2}{*}{+23.7} \\ 
%  &  & Ours & \textbf{43.4} & \textbf{73.2} \\ \cmidrule(l){2-6}
% & \multirow{2}{*}{16} & TSN & 19.9 & 47.3 & \multirow{2}{*}{+24.9}  \\ 
%  &  & Ours & \textbf{44.8} & \textbf{74.5} \\  \midrule
% % Something V2
% % TRN_somethingv2_RGB_resnet50_avg_segment3_e25
% \multirow{4}{*}{\shortstack{Something\\V2}} & \multirow{2}{*}{8} &  TSN & 27.8 & 57.6 & \multirow{2}{*}{+28.9}\\ 
% % TRN_somethingv2_RGB_resnet50_shift_shift8_blockres_avg_segment8_e50_nonflip_tunekk
%  &  & Ours & \textbf{56.7} & \textbf{83.7} \\ \cmidrule(l){2-6}
% & \multirow{2}{*}{16} & TSN & 30.0 & 60.5 &  \multirow{2}{*}{+27.5}\\ 
%  &  & Ours & \textbf{57.5} & \textbf{84.6} \\  \midrule
%  % Jester
%  % TRN_jester_RGB_resnet50_avg_segment8_e25_tunekk
% \multirow{4}{*}{Jester} & \multirow{2}{*}{8} & TSN & 81.0 & 99.0 & \multirow{2}{*}{+13.4} \\ 
% % TRN_jester_RGB_resnet50_shift_shift8_blockres_avg_segment8_e25_tunek
%  &  & Ours & \textbf{94.4} & \textbf{99.7} \\ \cmidrule(l){2-6}
% & \multirow{2}{*}{16} & TSN & 82.3 & 99.2 & \multirow{2}{*}{+13.0} \\ 
%  &  & Ours & \textbf{95.3} & \textbf{99.8} \\  
% \bottomrule
% \end{tabular} 
% \end{center}
% % \vspace{-20pt}
% \end{table}


\renewcommand \arraystretch{1}
\begin{table}[t]
%\setlength{\tabcolsep}{3pt}
\caption{Our method consistently outperforms 2D counterparts on multiple datasets at zero extra cost. All the results are reported on the validation set using RGB modality. All the models use ResNet-50 backbone, with the same training protocol.}
% \vspace{-6pt}
\label{tab:compared_2d}
\small
\begin{center}
\begin{tabular}{cccccc}
\toprule
\textbf{Dataset} & \textbf{\#Frame}& \textbf{Model} &  \textbf{Acc1} &  \textbf{Acc5} &  \textbf{$\Delta$ Acc1}  \\ 
\toprule
% Kinetics
\multirow{4}{*}{Kinetics} & \multirow{2}{*}{8} & TSN & 70.6 & 89.2 & \multirow{2}{*}{+3.5}  \\ 
% TRN_kinetics_RGB_resnet50_shift_shift8_blockres_avg_segment8_e45_tunek
 &  & Ours & \textbf{74.1} & \textbf{91.2} \\ \cmidrule(l){2-6}
& \multirow{2}{*}{16} & TSN & 70.7 & 89.2  & \multirow{2}{*}{+4.0} \\ 
% TSM_kinetics_RGB_resnet50_shift8_blockres_avg_segment16_e13_nopbn_dense
 &  & Ours & \textbf{74.7} & \textbf{91.4} \\  \midrule
% UCF-101
% TRN_ucf101_RGB_resnet50_avg_segment8_e25_tunekk
\multirow{4}{*}{UCF101} & \multirow{2}{*}{8} & TSN & 91.7 &  99.2& \multirow{2}{*}{+3.8} \\ 
% TRN_ucf101_RGB_resnet50_shift_shift8_blockres_avg_segment8_e25_tunekk
 &  & Ours & \textbf{95.5} & \textbf{99.6} \\ \cmidrule(l){2-6}
& \multirow{2}{*}{16} & TSN & 91.7 & 99.2& \multirow{2}{*}{+4.3}  \\ 
 &  & Ours & \textbf{96.0} & \textbf{99.6} \\  \midrule
% HMDB 
\multirow{4}{*}{HMDB51} & \multirow{2}{*}{8} & TSN & 64.7 & 89.9 & \multirow{2}{*}{+8.4} \\ 
 &  & Ours & \textbf{73.1} & \textbf{93.6} & \\ \cmidrule(l){2-6}
& \multirow{2}{*}{16} & TSN & 65.1 & 89.9 & \multirow{2}{*}{+8.1} \\ 
 &  & Ours & \textbf{73.2} & \textbf{93.9} \\   
\midrule \midrule
% ========================= Use 256x256 and 3 crop =====================
% --full_res --test_crops=3 --twice_sample
% Something V1 
\multirow{4}{*}{\shortstack{Something\\V1}} & \multirow{2}{*}{8} & TSN & 20.5  & 47.5 & \multirow{2}{*}{+24.6} \\ 
 &  & Ours & \textbf{45.1} & \textbf{74.0} \\ \cmidrule(l){2-6}
& \multirow{2}{*}{16} & TSN & 20.4 & 48.1 & \multirow{2}{*}{+25.1}  \\ 
 &  & Ours & \textbf{45.5} & \textbf{75.4} \\  \midrule
% Something V2
% TRN_somethingv2_RGB_resnet50_avg_segment3_e25
\multirow{4}{*}{\shortstack{Something\\V2}} & \multirow{2}{*}{8} &  TSN & 30.4 & 61.0 & \multirow{2}{*}{+28.7}\\ 
% TRN_somethingv2_RGB_resnet50_shift_shift8_blockres_avg_segment8_e50_nonflip_tunekk
 &  & Ours & \textbf{59.1} & \textbf{85.6} \\ \cmidrule(l){2-6}
& \multirow{2}{*}{16} & TSN & 30.5 & 61.2 &  \multirow{2}{*}{+28.9}\\ 
 &  & Ours & \textbf{59.4} & \textbf{86.1} \\  \midrule
 % Jester
 % TRN_jester_RGB_resnet50_avg_segment8_e25_tunekk
\multirow{4}{*}{Jester} & \multirow{2}{*}{8} & TSN & 83.9 & 99.6 & \multirow{2}{*}{+12.1} \\ 
% TRN_jester_RGB_resnet50_shift_shift8_blockres_avg_segment8_e25_tunek
 &  & Ours & \textbf{96.0} & \textbf{99.9} \\ \cmidrule(l){2-6}
& \multirow{2}{*}{16} & TSN & 84.6 & 99.6 & \multirow{2}{*}{+11.7} \\ 
 &  & Ours & \textbf{96.3} & \textbf{99.9} \\  
\bottomrule
\end{tabular}
\end{center}
% \vspace{-20pt}
\end{table}

==> figureText/tab_compare_2d_new.tex <==
% \renewcommand \arraystretch{1}
% \begin{table}[t]
% \caption{Our method consistently outperforms 2D counterparts on multiple datasets at zero extra cost. All the models use ResNet-50 backbone, with the same training protocol.}
% % \vspace{-6pt}
% \label{tab:compared_2d}
% \small
% \begin{center}
% \begin{tabular}{cccccc}
% \toprule
% & \textbf{Dataset} &  \textbf{Model} &  \textbf{Acc1} &  \textbf{Acc5} &  \textbf{$\Delta$ Acc1}  \\ 
% \toprule
% % Kinetics
% \multirow{6}{*}{\rotatebox{90}{Less Temporal\quad}} & \multirow{2}{*}{Kinetics} &  TSN & 70.6 & 89.2 & \multirow{2}{*}{+3.5}  \\ 
% % TRN_kinetics_RGB_resnet50_shift_shift8_blockres_avg_segment8_e45_tunek
%  &  & Ours & \textbf{74.1} & \textbf{91.2} \\ \cmidrule(l){2-6}
% % UCF-101
% % TRN_ucf101_RGB_resnet50_avg_segment8_e25_tunekk
% & \multirow{2}{*}{UCF101}  & TSN & 91.7 &  99.2& \multirow{2}{*}{+3.8} \\ 
% % TRN_ucf101_RGB_resnet50_shift_shift8_blockres_avg_segment8_e25_tunekk
%  &  & Ours & \textbf{95.5} & \textbf{99.6} \\ \cmidrule(l){2-6}
% % HMDB 
% & \multirow{2}{*}{HMDB51}  & TSN & 64.7 & 89.9 & \multirow{2}{*}{+8.4} \\ 
%  &  & Ours & \textbf{73.1} & \textbf{93.6} & \\ 
% \midrule \midrule
% % ========================= Use 256x256 and 3 crop =====================
% % --full_res --test_crops=3 --twice_sample
% % Something V1 
% \multirow{6}{*}{\rotatebox{90}{More Temporal\quad}}  & \multirow{2}{*}{\shortstack{Something\\V1}}  & TSN & 20.5  & 47.5 & \multirow{2}{*}{+24.6} \\ 
%  &  & Ours & \textbf{45.1} & \textbf{74.0} \\ \cmidrule(l){2-6}
% % Something V2
% % TRN_somethingv2_RGB_resnet50_avg_segment3_e25
% & \multirow{2}{*}{\shortstack{Something\\V2}}  &  TSN & 30.4 & 61.0 & \multirow{2}{*}{+28.7}\\ 
% % TRN_somethingv2_RGB_resnet50_shift_shift8_blockres_avg_segment8_e50_nonflip_tunekk
%  &  & Ours & \textbf{59.1} & \textbf{85.6} \\ \cmidrule(l){2-6}
%  % Jester
%  % TRN_jester_RGB_resnet50_avg_segment8_e25_tunekk
% & \multirow{2}{*}{Jester}  & TSN & 83.9 & 99.6 & \multirow{2}{*}{+12.1} \\ 
% % TRN_jester_RGB_resnet50_shift_shift8_blockres_avg_segment8_e25_tunek
%  &  & Ours & \textbf{96.0} & \textbf{99.9} \\ 
% \bottomrule
% \end{tabular}
% \end{center}
% % \vspace{-20pt}
% \end{table}

\renewcommand \arraystretch{1}
\begin{table}[t]
\caption{Our method consistently outperforms 2D counterparts on multiple datasets at zero extra computation. All the models use ResNet-50 backbone, with the same training protocol.}
% \vspace{-6pt}
\label{tab:compared_2d}
\small
\begin{center}
\begin{tabular}{cccccc}
\toprule
& \textbf{Dataset} &  \textbf{Model} &  \textbf{Acc1} &  \textbf{Acc5} &  \textbf{$\Delta$ Acc1}  \\ 
\toprule
% Kinetics
\multirow{6}{*}{\rotatebox{90}{Less Temporal\quad}} & \multirow{2}{*}{Kinetics} &  TSN & 70.7 & 89.2 & \multirow{2}{*}{+4.0}  \\ 
% TRN_kinetics_RGB_resnet50_shift_shift8_blockres_avg_segment8_e45_tunek
 &  & Ours & \textbf{74.7} & \textbf{91.4} \\ \cmidrule(l){2-6}
% UCF-101
% TRN_ucf101_RGB_resnet50_avg_segment8_e25_tunekk
& \multirow{2}{*}{UCF101}  & TSN & 91.7 &  99.2& \multirow{2}{*}{+4.3} \\ 
% TRN_ucf101_RGB_resnet50_shift_shift8_blockres_avg_segment8_e25_tunekk
 &  & Ours & \textbf{96.0} & \textbf{99.6} \\ \cmidrule(l){2-6}
% HMDB 
& \multirow{2}{*}{HMDB51}  & TSN & 65.1 & 89.9 & \multirow{2}{*}{+8.4} \\ 
 &  & Ours & \textbf{73.2} & \textbf{93.9} & \\ 
\midrule \midrule
% ========================= Use 256x256 and 3 crop =====================
% --full_res --test_crops=3 --twice_sample
% Something V1 
\multirow{6}{*}{\rotatebox{90}{More Temporal\quad}}  & \multirow{2}{*}{\shortstack{Something\\V1}}  & TSN & 20.4  & 48.1 & \multirow{2}{*}{+26.8} \\ 
 &  & Ours & \textbf{48.4} & \textbf{78.1} \\ \cmidrule(l){2-6}
% Something V2
% TRN_somethingv2_RGB_resnet50_avg_segment3_e25
& \multirow{2}{*}{\shortstack{Something\\V2}}  &  TSN & 30.5 & 61.2 & \multirow{2}{*}{+}\\ 
% TRN_somethingv2_RGB_resnet50_shift_shift8_blockres_avg_segment8_e50_nonflip_tunekk
 &  & Ours & \textbf{59.4} & \textbf{86.1} \\ \cmidrule(l){2-6}
 % Jester
 % TRN_jester_RGB_resnet50_avg_segment8_e25_tunekk
& \multirow{2}{*}{Jester}  & TSN & 84.6 & 99.6 & \multirow{2}{*}{+13.1} \\ 
% TRN_jester_RGB_resnet50_shift_shift8_blockres_avg_segment8_e25_tunek
 &  & Ours & \textbf{96.3} & \textbf{99.9} \\ 
\bottomrule
\end{tabular}
\end{center}
% \vspace{-15pt}
\end{table}

==> figureText/tab_compare_online_methods.tex <==
\renewcommand \arraystretch{1.1}
\begin{table}[t]
% \vspace{-10pt}
\small
\setlength{\tabcolsep}{3pt}
\caption{Compare the property of different online recognition methods.}
\label{tab:compare_online}
\small
\begin{center}
\begin{tabular}{ccccc}
\toprule
\textbf{Model} &
 \textbf{Low Lat.} & \textbf{Low Mem.} &  \textbf{Tepmral Fusion} & \textbf{Sth Acc.} \\ \midrule
TSN & \checkmark & \checkmark & No & 19.7 \\
TRN &  \checkmark & \checkmark & Final & 38.9  \\
ECO &   & & Middle & 39.6  \\
\midrule
TSM &  \checkmark & \checkmark  & Full & 42.0 \\
\bottomrule
\end{tabular}
\end{center}
% % \vspace{-17pt}
\end{table}

==> figureText/tab_inplace_vs_residual.tex <==
% \renewcommand \arraystretch{1}
% \begin{table}[t]
% \small
% \setlength{\tabcolsep}{9pt}
% \caption{Residual shift is better than in-place shift. In-place shift will harm the model capacity on spatial feature learning. Residual shift can balance between the spatial and temporal feature extraction. The performance is evaluated on the validation set of Kinetics.}
% \label{tab:inplace_vs_residual}
% \small
% \begin{center}
% \begin{tabular}{cccc}
% \toprule
% \textbf{Architecture}
% & \textbf{Proportion} & \textbf{Acc-1} & \textbf{Acc-5} \\ 
% \toprule
% % TSN baseline & - & 68.8 & 88.3 \\ \midrule
% TSN baseline & - & 70.6 & 89.2 \\ \midrule
% % \multirow{2}{*}{In-place shift} & 1/4 & 69.7 & 89.3 \\ 
% \multirow{2}{*}{In-place shift} & 1/4 & 73.2 & 91.0 \\ 
% % TRN_kinetics_RGB_resnet50_shift_shift4_block_avg_segment8_e30_tunek
% %  & 1/2 & 67.8 & 88.3 \\ \midrule
%  & 1/2 & 71.3 & 90.0 \\ \midrule
% % TRN_kinetics_RGB_resnet50_shift_shift16_blockres_avg_segment8_e30_tunek_cont
% % \multirow{3}{*}{Residual shift} & 1/8 & 70.4 & \textbf{89.6}\\
% \multirow{3}{*}{Residual shift} & 1/8 & 73.9 & \textbf{91.3}\\
% % TRN_kinetics_RGB_resnet50_shift_shift8_blockres_avg_segment8_e45_tunek
% % & 1/4 & \textbf{70.6} & 89.5 \\ 
% & 1/4 & \textbf{74.1} & 91.2 \\ 
% % TRN_kinetics_RGB_resnet50_shift_shift4_blockres_avg_segment8_e30_tunek_cont
% % & 1/2 & 69.9 & 89.7 \\ 
% & 1/2 & 73.4 & 91.1 \\ 
% \bottomrule
% \end{tabular}
% \end{center}
% % \vspace{-12pt}
% \end{table}


\renewcommand \arraystretch{1}
\begin{table}[t]
\small
\setlength{\tabcolsep}{4pt}
\caption{Residual shift is better than in-place shift. In-place shift will harm the model capacity on spatial feature learning. Residual shift can balance between the spatial and temporal feature extraction. The performance is evaluated on the validation set of Kinetics.}
\label{tab:inplace_vs_residual}
\small
\begin{center}
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}
& \multirow{2}{*}{\textbf{Ratio}} & \multirow{2}{*}{\textbf{Acc1}} & \multirow{2}{*}{\textbf{Acc5}} & \multirow{2}{*}{\textbf{\shortstack{Mem.\\Move\\(M)}}} & \multicolumn{3}{c}{\textbf{Device Latency (ms)}}  \\ 
\cmidrule(lr){6-8}
& & & & & P100 & TX2 & CPU \\
\toprule
% TSN baseline & - & 68.8 & 88.3 \\ \midrule
TSN & - & 70.7 & 89.2 & - \\ \midrule
% \multirow{2}{*}{In-place shift} & 1/4 & 69.7 & 89.3 \\ 
\multirow{3}{*}{\shortstack{In-place\\TSM}} & 1/4 & 73.8 & 91.2 & 11.2 \\ 
% TRN_kinetics_RGB_resnet50_shift_shift4_block_avg_segment8_e30_tunek
%  & 1/2 & 67.8 & 88.3 \\ \midrule
 & 1/2 & 71.9 & 90.2 & 22.5 \\ 
 & 1 &  & & 45.0 \\ 
 \midrule
% TRN_kinetics_RGB_resnet50_shift_shift16_blockres_avg_segment8_e30_tunek_cont
% \multirow{3}{*}{Residual shift} & 1/8 & 70.4 & \textbf{89.6}\\
\multirow{4}{*}{\shortstack{Residual\\TSM}} & 1/8 & 74.5 & \textbf{91.5} & 5.6\\
% TRN_kinetics_RGB_resnet50_shift_shift8_blockres_avg_segment8_e45_tunek
% & 1/4 & \textbf{70.6} & 89.5 \\ 
& 1/4 & \textbf{74.7} & 91.4 & 11.2 \\ 
% TRN_kinetics_RGB_resnet50_shift_shift4_blockres_avg_segment8_e30_tunek_cont
% & 1/2 & 69.9 & 89.7 \\ 
& 1/2 & 74.0 & 91.3 & 22.5 \\ 
 & 1 &  &  & 45.0 \\ 
\bottomrule
\end{tabular}
\end{center}
% \vspace{-10pt}
\end{table}

==> figureText/tab_online_ablation.tex <==
\renewcommand \arraystretch{1.1}
\begin{table}[t]
% \vspace{-10pt}
\small
\setlength{\tabcolsep}{5pt}
\caption{Ablation study of online video recognition with TSM.}
\label{tab:online_ablation}
\small
\begin{center}
\begin{tabular}{cccc}
\toprule
\textbf{Offline TSM} &
 \textbf{Online TSM} & \textbf{Final Fusion} & \textbf{Sth Acc.} \\ \midrule
 &  &  & 19.7 \\ 
 \midrule
 \checkmark &  &  & \textbf{43.4} \\ 
%  \midrule
 &  \checkmark  &  & 42.0 \\ 
%   \midrule
  &   &  \checkmark & 39.6 \\ 
%   \midrule
   & \checkmark  &  \checkmark & \textbf{43.4} \\ 
\bottomrule

\end{tabular}
\end{center}
% \vspace{-17pt}
\end{table}

==> figureText/tab_padding.tex <==
\renewcommand \arraystretch{1.}
\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\caption{Zero padding is better than circulant padding. }
\label{tab:padding}
\small
\begin{center}
\begin{tabular}{ccc}
\toprule
\textbf{Padding Type}
& \textbf{Kinetics Acc.} & \textbf{Something Acc.}\\ 
\toprule
% TRN_something_RGB_resnet50_avg_segment8_e25_nonflip_tunek
% TSN baseline & 68.8 & 19.7 \\ \midrule
TSN baseline & 70.6 & 20.5 \\ \midrule
% TRN_kinetics_RGB_resnet50_shift_shift8_blockres_avg_segment3_e45_nopbn
% TRN_something_RGB_resnet50_shift_shift8_blockres_avg_segment8_e50_nonflip_tunek
% Zero & \textbf{70.6} & \textbf{43.4} \\ 
Zero & \textbf{74.1} & \textbf{45.1} \\ 
% TRN_kinetics_RGB_resnet50_shift_circshift8_blockres_avg_segment3_e45_tunek
% TRN_something_RGB_resnet50_shift_circshift8_blockres_avg_segment8_e50_nonflip_tunek
% Circulant & 69.5 & 40.8 \\
Circulant & 73.0 & - \\
\bottomrule
\end{tabular}
\end{center}
% % % \vspace{-15pt}
\end{table}

==> figureText/tab_vs_nonlocal.tex <==
\renewcommand \arraystretch{1.}
\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\caption{Our TSM model can be combined with other techniques like Non-local~\cite{wang2017non} module. Accuracy measured on Kinetics dataset with ResNet-50 backbone with 5 NL blocks. We replaced the 3D convolution in~\cite{wang2017non} with TSM while keeping network architecture and training protocol the same.}
\label{tab:vs_nonlocal}
\small
\begin{center}
\begin{tabular}{ccc}
\toprule
\textbf{Model}
& \textbf{top-1} & \textbf{top-5}  \\ 
\toprule
I3D & 73.3 & 90.7  \\ 
TSM & &  \\ 
\midrule
NL I3D  & 74.9 & 91.6 \\
NL TSM  &  & \\
\bottomrule
\end{tabular}
\end{center}
% \vspace{-15pt}
\end{table}

==> text/9_acknowledge.tex <==
\paragraph{Acknowledgments}
We thank MIT Quest for Intelligence, MIT-IBM Watson AI Lab, Samsung, SONY, AWS, Google for supporting this research. We thank Oak Ridge National Lab for Summit supercomputer.


==> text/approach.tex <==
\section{Approach}

In this section, we will first describe the \method Module (TSM) for temporal modeling, and then show how we use it to build the \emph{\netFull video model} for efficient long-term video understanding.

\input{figureText/fig_overall}


\subsection{Intuition}
For a video understanding framework, the shape of activation is usually $[N, C, T, H, W]$ (activation $A\in\mathbb{R}^{N\times C\times T\times H\times W}$), where $N$ is the batch size, $C$ is the number of channels, $T$ is the temporal dimension, $H$ and $W$ are the spatial resolutions. 

% For an input RGB image we have $C=3$. 
% \SH{below is not our work, can be moved to background or removed}
% 2D convolutional networks based frameworks like TSN~\cite{wang2016temporal} processes the images of different time stamps independently without temporal fusion. Such methods regard the tensor as a batch of $N\times T$ samples with shape $[N\times T, C, H, W]$ and run the 2D CNN for $N\times T$ samples respectively, without effective temporal modeling.
% % thus no information exchange happens during inference until the very end. Therefore such methods do not allow complex temporal modeling, as much of the information is lost during inference.
% 3D convolutional neural network based methods like C3D~\cite{tran2015learning} and I3D~\cite{carreira2017quo} jointly convolve across spatial and temporal dimension, progressively fusing the temporal information between frames, thus prove to be more effective on datasets where temporal modeling is critical~\cite{goyal2017something, jester, sigurdsson2016hollywood}.
% However, the massive amount of computational has limited their applications on edge devices.

% In this paper, we address the computational cost and temporal modeling ability dilemma by proposing a novel \textbf{\method} module, which is able to handle highly complicated temporal relationship at \textbf{zero cost}: zero extra FLOPs and zero extra parameters. 

Let us first consider a normal convolution operation. For brevity, we used a 1-D convolution with the kernel size of 3 as an example. Suppose the weight of the convolution is $W=(w_1, w_2, w_3)$, and the input $X$ is a 1-D vector with infinite length. The convolution operator $Y=\text{Conv}(W, X)$ can be written as:
$ Y_i =  w_1 X_{i-1} + w_2 X_{i} + w_3 X_{i+1}$.
We can decouple the operation of convolution into two steps: \emph{shift} and \emph{multiply-accumulate}: we shift the input $X$ by $-1, 0, +1$ and multiply by $w_1, w_2, w_3$ respectively, which sum up to be $Y$. Formally, the \emph{shift} operation is:
% \begin{equation}
% \begin{split}
%     X^{-1}_i &= X_{i-1}, \\
%     X^{0}_i &= X_i, \\ 
%     X^{+1}_i &= x_{i+1}, \\
% \end{split}
% \end{equation}
\begin{equation}
    X^{-1}_i = X_{i-1},~~~~ X^{0}_i = X_i, ~~~~ X^{+1}_i = x_{i+1}
\end{equation}
and the \emph{multiply-accumulate} operation is:
\begin{equation}
    Y=w_1 X^{-1} + w_2 X^{0} + w_3 X^{+1}
\end{equation}
The first step \emph{shift} can be conducted at no computational cost. While the second step is more computationally expensive, our \method module \emph{merges} the \emph{multiply-accumulate} into the following 2D convolution, so 
% that we can build a network to model temporal information but 
it introduces no extra cost compared to 2D CNN based models.


\input{figureText/fig_shift_place}

\subsection{Temporal Shift Module}
Our proposed \method module is described in Figure~\ref{fig:shift}. For brevity, we only show the temporal $T$ and channel $C$ dimensions, while dropping batch size $N$, height $H$, and width $W$, since they are not related to our discussion. In Figure~\ref{fig:shift_ori}, we describe a tensor with $C$ channels and $T$ frames. The features at different time stamps are denoted as different colors in each row. Conventional 2D CNN operates among channels, that is to operate along each row separately without temporal fusion.

% As the 2-step decomposition of convolution mentioned above, we apply the first step of decomposition \emph{shift} to the temporal dimension. For example, here we simulate a convolution with kernel size 3 in Figure.

Along the temporal dimension, we shift one-quarter channels by $-1$, another quarter by $+1$, leaving the rest half un-shifted (Figure~\ref{fig:shift_zero}). ``A quarter" is a hyperparameter we will discuss in the ablation study (Section~\ref{sec:appr_variant}). Which quarter to shift doesn't matter since the weights in the next layer will adapt to it during training.  As a result, we mingle the temporal information from frame $t-1$, $t$, and $t+1$ together, similar to a 1D convolution with the kernel size of 3, but at zero computation cost. The \emph{multiply-accumulate} is pushed to the next layer. It borrows the 2D convolution's inter-channel fusion ability to perform the original inter-temporal fusion.

% After the first step \emph{shift}, we need to incorporate the second step \emph{multiply-accumulate} into existing 2D CNN backbone. The section of channels to shift are manually assigned, but luckily, in convolutional neural networks, the convolution layers operate densely from input channels to output channels. So if the \method module is followed by a normal convolutional layer, the shifted channels will be fused by the convolution, in an end-to-end learn-able way. Furthermore, after temporal shifting, the different channels (\ie, a row in the figure) for an image at a certain time stamp now contains original channels from different time stamps, thus we can borrow the 2D convolution's inter-channels fusion ability to perform the original inter-temporal fusion. In such way, we successfully incorporate the second step \emph{multiply-accumulate} on temporal dimension into the existing 2D CNN backbone.


\subsection{Variant of \method} \label{sec:appr_variant}

Here we describe the several variants of implementing our proposed \method module.



\myparagraph{In-place shift or residual shift.}
% One possible drawback of the \method module is that the information about current frame stored in the shifted channels is lost for the following 2D CNN. 
A straightforward way to apply our \method module is to insert it before each convolutional layer or residual block, as illustrated in Figure~\ref{fig:shift_inplace}. We call such \method module directly inserted before a convolution layer \emph{in-place shift}.

One possible drawback of the \emph{in-place shift} is the loss of spatial feature learning capability. After temporal shift, part of the information stored in the shifted channels is lost for the current frame.
It could be a problem if we shift too many channels, \eg, $1/2$ (ablation study in Section~\ref{sec:exp_ablation}). 
To address such issue, we propose a variant of the shift module. Instead of inserting it in-place, we put the temporal shift module \emph{inside} the residual branch in a residual layer, so that the information inside the shifted channels will still be available through identity mapping. We denote such version of shift as \emph{residual shift}. Experiments show that residual based temporal shift achieves better performance compared to its in-place counterparts and is less sensitive to the proportion. Meanwhile, it does not harm the spatial features learning while learning temporal features.

\myparagraph{Zero padding or circulant padding.}
As illustrated in Figure~\ref{fig:shift}, after temporal shifting, there will be empty channels at the boundary. We need to pad the empty boundary. The straightforward idea is to pad the empty space with zeros. The extra channels can be shifted out and truncated.

Another padding strategy is to use a circulant padding scheme, \ie, the shifted-out channels are used to fill the corresponding empty spaces. However, the temporal order will be broken after circulant padding: the channel in the later frames will be shifted to the front of the early ones. Such padding strategy harms the temporal modeling performance. We verified this phenomenon in the ablation study (Section~\ref{sec:exp_ablation}).

% \textbf{Kernel of Shift}. 
% In Figure~\ref{fig:shift_zero}, we present an example of temporal shifting with kernel (-1, 0, +1), \ie, part of the channels are shifted by 1 time stamp along temporal axis and vice versa. Since the shift operation itself is of no cost, we can easily adjust the kernel of temporal shift to achieve a larger temporal perceptive field. For example, we can use a larger kernel (-2, -1, 0, +1, +2) or a strided one (-2, 0, +2).


\subsection{\netFull Video Models} \label{sec: shift-3d model}




In this section, we describe how to leverage the proposed \method module to build a video recognition model based on purely 2D CNNs without any extra cost.

% \myparagraph{Frame sampling.} A raw video $V$ usually consists of hundreds or thousands of frames with a high frame rate, which are redundant and too heavy to perform per frame inference. Thus video understanding models begin with frame sampling. Existing frame sampling strategy can be roughly divided into two categories: dense sampling~\cite{tran2015learning, carreira2017quo, wang2017non, xie2018rethinking} and strided sampling~\cite{wang2016temporal, zhou2017temporal, zolfaghari2018eco}. 
% To build an efficient model, we use strided sampling strategy which first divides the whole video into $N$ sections of equal size $S_i, i=1, 2, ..., N$, and samples one frame per section, same for training and testing. Another advantage of strided sampling is that it covers the whole video instead of a local subset; thus it is better for long-term temporal modeling. 
% Since we want to build an efficient video network, we adopt the strided sampling strategy, so that the model does not need to exhaustively access all the frames.

% \myparagraph{2D CNN baselines (C2D/TSN).}
% After frame sampling, 2D CNN baselines inference on each of the frames individually, and the output logits are averaged to give the final prediction. No temporal fusion is conducted during the process until the very end.

% \myparagraph{\netFull Video Model.}
Given a raw video $V$, we first sample $T$ frames $F_i, F_1, ..., F_T$ from the video.
Then we adopt a 2D CNN baselines to process each of the frames individually, and the output logits are averaged to give the final prediction. 
% No temporal fusion is conducted during the process until the very end.
Our proposed \netFull model is largely based on the corresponding 2D CNN baseline, with exactly the same parameters and computation cost. During most of the inference process like convolution layers, the frames are still running independently, just like the 2D CNNs. The difference is that for \netFull models, temporal shift module is inserted for each layer/residual unit, which enables temporal information fusion at no cost.
For each inserted temporal shift module, the temporal receptive field will be enlarged by 2, as if running a convolution with the kernel size of 3 along the temporal dimension. Therefore, our \netFull model has a very large temporal receptive field to conduct highly complicated temporal modeling.

A unique advantage of our method is that we can easily convert any off-the-shelf 2D CNN model into a pseudo-3D model that can handle both spatial and temporal information, without adding additional cost. Thus the deployment of our framework is hardware friendly: we only need to support the operations in 2D CNNs, which are already well-optimized at both framework level (CuDNN~\cite{chetlur2014cudnn}, MKL-DNN) and hardware level (CPU/GPU/TPU/FPGA).
% \SH{can add citation}

% \SH{can delete Temporal Pooling if overflow}
% \myparagraph{Better Efficiency by Temporal Pooling.}
The computation cost grows linearly with the number of frames. Previous methods~\cite{tran2015learning, carreira2017quo, wang2017non, wang2018videos, xie2018rethinking} widely used temporal max pooling to reduce the temporal dimension during inference, which effectively reduces the computational cost of the network. We also used a similar technique here by inserting a max pooling layer between the first and the second residual layer. We use the kernel size of 3 and the stride of 2 for the temporal max pooling module. We denote the model without temporal pooling as \textbf{\netFull}, and the model with temporal pooling as \textbf{\netFull-P}.

\subsection{Online Recognition with Single-sided TSM}
\input{figureText/fig_singlesided}

Online and low-latency video recognition is of vital significance for real-life deployment. 
3D based spatio-temporal networks are by nature offline models. Some works like~\citep{zolfaghari2018eco} combines early 2D CNN for feature extraction and late 3D CNN for temporal modeling. However, Applying 3D CNN over multiple frames is still computational extensive, which increases the latency of video recognition.

Here we show that by modifying TSM to shift single-sided, \ie, only shift part of the features from last timestamp to current frame, we can enable efficient and high-performance online video understanding. 
% For an online video stream $..., I_{t-1}, I_t, I_{t+1}, ...$, online recognition requires us to give a per-frame prediction with minimum latency. 
As shown in Figure~\ref{fig:singlesided}, given a frame $I_t$, single-sided TSM only shifts out a small fraction of feature maps (\eg, $\frac{1}{8}$) and store them in the memory. We denote the shifted channels as $\lbrace S_{t}^{i}\rbrace$, where $i$ is the layer index. The shifted out channels are replaced with the shifted channels $\lbrace S_{t-1}^{i}\rbrace$ from last frame $I_{t-1}$. The shift-and-replace operation operates in a recursive way. 

The single-sided TSM is also very efficient for online video recognition. For computation, single TSM brings no extra FLOPs;
For memory consumption, we only need to shift out and cache a very small fraction of feature maps. For example, adding online TSM to ResNet-50 requires around \textbf{[TODO]} MB memory cache.
%The size of the cached feature maps is even smaller when we added TSM in the bottleneck as in Figure~\ref{fig:shift_bottleneck}.

==> text/offline.tex <==
\section{Offline TSM Networks} \label{sec: offline}

Although our proposed TSM can support online video recognition, we first test our offline version TSM as most of the state-of-the-art results are obtained from offline models~\cite{carreira2017quo, wang2017non}. We hope to compare with the state-of-the-art results to show the temporal modeling ability of our TSM module. 

\subsection{Building Spatio-temporal Networks with TSM}
Given a raw video $V$, we first sample $T$ frames $F_i, F_1, ..., F_T$ from the video.
After frame sampling, 2D CNN baselines process each of the frames individually, and the output logits are averaged to give the final prediction. 
% No temporal fusion is conducted during the process until the very end.
Our proposed \netFull model is largely based on the corresponding 2D CNN baseline, with exactly the same parameters and computation cost. During most of the inference process like convolution layers, the frames are still running independently, just like the 2D CNNs. The difference is that for \netFull models, temporal shift module is inserted for each layer/residual block, which enables temporal information fusion at no cost.
For each inserted temporal shift module, the temporal receptive field will be enlarged by 2, as if running a convolution with the kernel size of 3 along the temporal dimension. Therefore, our \netFull model has a very large temporal receptive field to conduct highly complicated temporal modeling. In this paper, we used \textit{ResNet-50}~\cite{he2016deep} as the backbone for all the experiments unless otherwise specified.

A unique advantage of our method is that we can easily convert any off-the-shelf 2D CNN model into a pseudo-3D model that can handle both spatial and temporal information, without adding additional cost. Thus the deployment of our framework is hardware friendly: we only need to support the operations in 2D CNNs, which are already well-optimized at both framework level (CuDNN~\cite{chetlur2014cudnn}, MKL-DNN) and hardware level (CPU/GPU/TPU/FPGA).
% \SH{can add citation}

% \SH{can delete Temporal Pooling if overflow}
% \myparagraph{Better Efficiency by Temporal Pooling.}
The computation cost grows linearly with the number of frames. Previous methods~\cite{tran2015learning, carreira2017quo, wang2017non, wang2018videos, xie2018rethinking} widely used temporal max pooling to reduce the temporal dimension during inference, which effectively reduces the computational cost of the network. We also used a similar technique here by inserting a max pooling layer between the first and the second residual layer. We use the kernel size of 3 and the stride of 2 for the temporal max pooling module. We denote the model without temporal pooling as \textbf{\netFull}, and the model with temporal pooling as \textbf{\netFull-P}.




\subsection{Improving 2D CNN Baselines}

We can seamlessly inject \method module into a normal 2D CNN  and improve its performance on video recognition. In this section, we demonstrate a 2D CNN baseline can significantly benefit from our \method module with double-digits accuracy improvement.  Here we aim to show the improvement over the baselines. We will demonstrate how to push it to the state-of-the-art in the next section. We used 8 sampled frames per video clip.
% (8/16 compared to 32/64 in other works), for the purpose of efficiency.

We chose TSN~\cite{wang2016temporal} as the 2D CNN baseline. We used the same training protocol for TSN and our \netFull. The only difference is whether our \method module is used or not.  The results on several action recognition datasets are listed in Table~\ref{tab:compared_2d}. The chart is split into two parts. The upper part contains datasets Kinetics~\cite{kay2017kinetics}, UCF101~\cite{soomro2012ucf101}, HMDB51~\cite{kuehne2011hmdb}, where temporal relationships are less important, while our \netFull still consistently outperforms the 2D TSN baseline at no extra cost. For the lower part, we present the results on Something-Something V1 and V2~\cite{goyal2017something} and Jester~\cite{jester}, which depend heavily on temporal relationships. TSN baseline cannot achieve a good accuracy, but once equipped with our \method module, the performance improved by double digits. For example, on Something-Something-V1 dataset, our \netFull achieves 24.6\% better performance than the 2D baseline, even though the computation costs of the two methods are exactly the same. 

\input{figureText/tab_compare_2d_new}

\subsection{Comparison with State-of-the-Arts}

\input{figureText/tab_compare_something}


\netFull can outperform state-of-the-art methods, which heavily rely on 3D convolutions. We compared the performance of our \netFull model with state-of-the-art methods on both Something-Something V1\&V2 because these two datasets focus on temporal modeling.

\myparagraph{Something-Something-V1.} 
% Something-Something-V1 is a challenging dataset, as activity cannot be inferred merely from individual frames (\eg, pushing something from \emph{right to left}, pushing something from \emph{left to right}, moving something \emph{up}). An individual frame can not differ \emph{left to right} and \emph{right to left}, or \emph{up} and \emph{down}. We compared the results of the proposed \netFull with current state-of-the-art methods on Something-Something-V1 in Table~\ref{tab:compare_something}. We only applied the center crop during testing to ensure the efficiency.

In Table~\ref{tab:compare_something} we first present the 2D based methods, including TSN~\cite{wang2016temporal} and TRN~\cite{zhou2017temporal}. The original results use BNInception as the backbone, we re-implement the experiments with ResNet-50 backbone, which achieves better performance.
TSN fails to achieve decent performance (19.7\%  Top-1), due to the lack of temporal modeling. For TRN, although \textbf{late temporal fusion} is added after feature extraction, the result is still significantly lower than state-of-the-art methods, showing the importance of early temporal fusion. 

The second section shows the state-of-the-art efficient video understanding framework ECO~\cite{zolfaghari2018eco}. 
ECO uses an early 2D + late 3D architecture which enables \textbf{medium-level temporal fusion}.
Compared to ECO, our method achieves better performance at a smaller FLOPs. For example, when using 16 frames as input, our \netFull-P achieves 43.8\% top-1 accuracy with 39G FLOPs, which is 2.4\% more accurate than ECO and 1.6$\times$ less computation. The ensemble versions of ECO (ECO\textsubscript{\emph{En}}\emph{Lite} and ECO\textsubscript{\emph{En}}\emph{Lite}\textsubscript{RGB+Flow}, using an ensemble of  \{16, 20, 24, 32\} frames as input) did achieve competitive results, but the computation and parameters are too large for deployment. While our model is much more efficient: we only used \{8, 16\} frames model for ensemble (\netHead\textsubscript{\emph{En}}), and the model achieves better performance using 2.7$\times$ less computation and 3.1$\times$ fewer  parameters.
% our model consumes 81.3\% less computation and 83.8\% less parameters compared to ensemble ECO while achieving even higher performance. 

The third section contains methods that achieve previous best performance on the leaderboard: Non-local I3D + GCN~\cite{wang2018videos}, that enables \textbf{all-level temporal fusion}. The GCN needs a Region Proposal Network~\cite{ren2015faster} trained on MSCOCO object detection dataset~\cite{lin2014microsoft} to generate the bounding boxes, which is unfair to compare since external data (MSCOCO) and extra training cost is introduced. Thus we compared \netFull to its CNN part: Non-local I3D. Our \netFull (16f) achieves 0.4\% better accuracy with $5\times$ fewer FLOPs on the validation set compared to the Non-local I3D network. Note that the NL I3D used in~\cite{wang2018videos} uses much more computation than the original NL I3D in~\cite{wang2017non}, which could be due to the fact the Something-Something datasets are more temporal related and thus needs more frames for recognition. 
Techniques like Non-local module~\cite{wang2017non} are orthogonal to our work, which could also be added to our framework to boost the performance further.


\myparagraph{Generalize to Other Modalities.} We also show that our proposed method can generalize to other modalities like optical flow. To extract the optical flow information between frames, we followed~\cite{wang2016temporal} to use the TVL1 optical flow algorithm~\cite{zach2007duality} implemented in OpenCV with CUDA. We conducted two-stream experiments on both Something-Something V1 and V2 datasets, and it consistently improves over the RGB performance: introducing optical flow branch brings 4.8\% top-1 improvement on both V1 and V2 evaluation sets. Our two-stream model achieves the \emph{current best result} on both Something-Something V1 and V2 leaderboard at the time of submission.

\myparagraph{Something-Something-V2.} We also show the result on Something-Something-V2 dataset, which is a newer release to its previous version, containing more videos for training. The results compared to other state-of-the-art methods are shown in Table~\ref{tab:somethingv2}. 
On Something-Something-V2 dataset, we achieved the best result on the leaderboard at the time of submission without bells and whistle, surpassing previous state-of-the-art result by 3.6\%. Note that the RGB input result of our model is only 0.2\% worse than previous state-of-the-art result using two-stream input, showing that our \netFull is strong at handling temporal modeling.


\input{figureText/tab_somethingv2}


\myparagraph{Cost \vs Accuracy.}
Our \netFull model achieves very competitive performance while enjoying high efficiency and low computation cost for fast inference. We show the FLOPs for each model in Table~\ref{tab:compare_something}. 
% For TRN~\cite{zhou2017temporal} and ECO~\cite{zolfaghari2018eco}, we measured the speed using the code released by the author. For I3D + GCN~\cite{wang2018videos}, we contacted author about the ones that cannot be inferred from the paper. 
Although GCN itself is light, the method used a ResNet-50 based Region Proposal Network~\cite{ren2015faster} to extract bounding boxes, whose cost is also considered in the chart.
% We can see that our \netFull is extremely efficient \wrt accuracy-computation trade-off. 
Note that in actual deployment we need to consider the computation cost of optical flow extraction, which is usually much larger than the video recognition model itself. Therefore, we do not report the FLOPs of two-stream based methods.


We show the accuracy, FLOPs, and number of parameters trade-off in Figure~\ref{fig:acc_vs_flops}. The accuracy is tested on the validation set of Something-Something-V1 dataset, and the number of parameters is indicated by the area of the circles. We can see that our \netFull based methods have a better Pareto curve than both previous state-of-the-art efficient models (ECO based models) and high-performance models (non-local I3D based models). 
% Moreover, efficient models like ECO has good computation-accuracy trade-off when the accuracy is not too high, but such property cannot be extended to state-of-the-art accuracy zone, leading to a worse trade-off.
Our \netFull models are both efficient and accurate. It can achieve state-of-the-art accuracy at high efficiency: it achieves better performance while consuming $3\times$ less computation than the ECO family and $6\times$ less computation than the Non-local I3D family. The model size is also $3\times$ smaller than ensemble ECO. Considering that ECO is already an efficiency-oriented design, our method enjoys highly competitive efficiency.
% it achieves 49.6\% top-1 accuracy at the cost of $1/5$ FLOPs and $1/5$ parameters compared to ensemble ECO.

\input{figureText/tab_runtime}

\subsection{Latency and Throughput Speedup}

% \renewcommand \arraystretch{1.2}
% \begin{table*}[t]
% \setlength{\tabcolsep}{3pt}
% \caption{Runtime analysis.}
% \label{tab:runtime}
% \small
% \begin{center}
% \begin{tabular}{cccccc|cccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} 
% &\multirow{2}{*}{\textbf{\shortstack{Sampled\\Frames}}}  & \multicolumn{4}{c}{\textbf{Statistics}} & \multicolumn{4}{c}{\textbf{Accuracy}} \\ 
% \cmidrule{3-10}
% & & Param. & FLOPs & Memory &  Video/s & UCF101 & HMDB51 & Kinetics & Something-V1 \\ 
% \toprule
% \multirow{2}{*}{ECO~\cite{zolfaghari2018eco}} & 8 & 33.7M & 25G & 495MB & 61 & 91.7 & 65.6 & 67.8 & 39.6 \\ 
%  & 16 & 34.1M & 50G & 723MB & 32 & 92.8 & 68.5 & 69.0 & 41.4 \\ \midrule
%  \multirow{2}{*}{\netFull-P} & 8 & \multirow{2}{*}{24.3M} & 19G & 184MB & 57 &  &  &   \\ 
%  & 16 &  & 39G & 274MB & 39 & &  &   & 43.8 \\ \midrule
%  % shift 3d
%   \multirow{2}{*}{\netFull} & 8 & \multirow{2}{*}{24.3M} & 33G & 199MB & 48 & 94.0 & 70.3 & 70.6 & 43.4 \\ 
%  & 16 &  & 65G & 1 & 31 & 94.5 & 70.7 & 72.5 & 44.8 \\ 
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table*}

The measured inference latency and throughput are important for the large-scale deployment of video understanding algorithms.
Our method has not only low FLOPs but also low latency and high throughput. We performed measurement on a single NVIDIA Tesla P100 GPU. We excluded the data loading time for fair comparison. To measure the latency, we used a batch size of 1; to measure the throughput, we used a batch size of 16. We first conducted warm-up inference for 100 runs and measured the averaged speed for 200 runs. The memory consumption was measured with PyTorch~\cite{paszke2017automatic}. 
% Although we can actually implement a temporal shift algorithm with zero cost using custom kernel, here we just use the naive split-pad-concat implementation. 
Compared with the popular I3D algorithm, our method achieved $8\times$ lower latency (20.7ms \vs 165.3ms), $12\times$ higher throughput (77 videos per second \vs 6 videos per second), $2.7\times$ smaller memory consumption (199MB \vs 540MB), at 1.8\% higher accuracy (Table~\ref{tab:runtime}). We also compared our method to the state-of-the-art efficient model ECO~\cite{zolfaghari2018eco}: Our \netFull-P model has $1.7\times$ lower latency (18.4ms \vs 30.6ms), $1.7\times$ higher throughput, less than half the memory consumption, and achieves 2\% better accuracy.  ECO has an expensive two-branch (2D+3D) architecture, while our method only needs the in-expensive 2D backbone.
Furthermore, the above results are based on a naive split-pad-concatenate implementation. We expect even higher speedup if we can implement a customized kernel for temporal shift. 

% \renewcommand \arraystretch{1.2}
% \begin{table}[t]
% \small
% \setlength{\tabcolsep}{3pt}
% \caption{Inference analysis. \netFull consistently outperforms ECO on Something-Something dataset, while consumes much less memory. The actual inference speed of our method is also very competitive: on 16 frame setting our \netFull-P is 19\% faster than ECO while achieves 2.4\% better accuracy. (Video/s higher the better.)  }
% \label{tab:runtime}
% \small
% \begin{center}
% \begin{tabular}{ccccccc}
% \toprule
% \textbf{Model} &
% \textbf{\shortstack{\#Fr}}  & \textbf{FLOPs} & \textbf{Memory} &  \textbf{Video/s} &\textbf{Sth Acc.} \\ \midrule
% \multirow{2}{*}{ECO~\cite{zolfaghari2018eco}} & 8  & 32G & 500MB & 61.2 & 39.6 \\ 
%  & 16  & 64G & 735MB & 32.7 & 41.4 \\ \midrule
%  \multirow{2}{*}{\netFull-P} & 8 &   19G & 199MB & 56.7 & 40.1 \\ 
%  & 16 & 39G & 301MB & 38.9 & 43.8 \\ \midrule
%  % shift 3d
%   \multirow{2}{*}{\netFull} & 8   & 33G & 199MB & 48.2 & 43.4 \\ 
%  & 16  & 65G & 301MB & 30.8 & 44.8  \\ 
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}



==> text/online.tex <==
\section{Online TSM Networks}

Video understanding from online video streams is very important in real-life scenarios. In this section, we show that we can modify our TSM to achieve online video recognition while with multi-level temporal fusion.

\subsection{Online Recognition with Single-sided TSM}

\input{figureText/fig_singlesided}

As shown in Figure~\ref{fig:shift}, offline TSM shifts part of the channels bi-directionally, which requires features from future frames to replace the features in the current frame. If we only shift the feature from previous frames to current frames, we can achieve online recognition with single-sided TSM.

We show the inference time graph of how to utilize single-sided TSM for online video recognition in Figure~\ref{fig:singlesided}. During inference, for each frame, we shift out parts of the features of different residual block and cache it in the memory. For the next frame, we replace the corresponding features with the cached features, and cache the replace features, and so on.

Using single-sided TSM fro online video recognition shares several unique advantages: 1. \textbf{Low latency inference}. For each frame, we only need to replace and cache some of the features, without incurring any extra computations. Therefore, the latency of per-frame prediction is almost the same as the 2D CNN baseline.  2. 
\textbf{Low memory consumption}. Since we only cache a small portion of the features in the memory, the memory consumption is low. For ResNet-50, we only need 3.8MB memory cache. 3. \textbf{Multi-level temporal fusion}. Most of the online method only enables final temporal fusion after feature extraction like~\cite{zhou2017temporal} or middle level temporal fusion~\cite{zolfaghari2018eco}. While  TSM enables all level temporal fusion.

% \input{figureText/tab_compare_online_methods}


\subsection{From Offline to Online Model}

\input{figureText/tab_online_vs_offline}
% \input{figureText/tab_online_ablation}


% According to our experiments, by replacing offline bi-directional TSM to online single-sided TSM, we can still achieve similar accuracy on less temporal-related datasets like Kinetics (offline 74.7\% v.s. online 74.8\%), while the performance drops on more temporal-related datasets like Something-Something. Therefore, we mainly study the accuracy on Something-Something dataset.

% We compare the performance of different version of TSM in Table~\ref{tab:online_ablation}. We find that online version of TSM can also significantly improve over the 2D baseline by 22.3\%, while introducing no extra computation for the prediction of each frame. However, online TSM achieves 1.4\% lower accuracy compared to offline TSM. We hypothesize that the performance drop comes from the lack of bi-directional temporal reasoning.
% To tackle the problem while maintain low-latency online prediction, we make the final block of ResNet shift bi-directionally, while keeping all the other layers shift single-sided. As the last block of ResNet only makes up \textbf{TODO\%} of the computation, the latency will not be largely increased. Such modification is denoted as \textbf{Final Fusion} in Table~\ref{tab:online_ablation}. We find that online TSM along with final fusion achieves the same performance as offline TSM, while providing low-latency online prediction. We also tried adding the final fusion alone, which only achieves 39.6\% accuracy. It again shows the importance of multi-level temporal fusion.

\myparagraph{Online \vs Offline}
Despite the real-time prediction ability of online TSM models, the accuracy could be hurt due to the lack of bi-directional temporal reasoning. Here we compare the performance of offline and online TSM models on video recognition tasks. Online video prediction model can give a prediction for each of the frames. To compare the performance with offline models, we use the prediction averaged from all the frames, \ie, we compare the performance after observing the whole videos. We use the same frame sampling strategy for both the online and offline models. The performance comparison is provided in Table~\ref{tab:offline_online}.
We can see that for less temporal related datasets like Kinetics, UCF101 and HMDB51, the online models achieve comparable and sometimes even better performance compared to the offline models. While for more temporal related datasets Something-Something, online model performs worse than offline model by 1.2\% due to the lack of bi-directional temporal reasoning. Nevertheless, the performance of online model is still significantly better than the 2D baseline.

We also compare the per-frame prediction latency of pure 2D backbone (TSN) and our online TSN model. Our online TSN model only adds to 0.6ms latency overhead per frame, while bringing considerable performance gain. Therefore, we believe that our online TSM module is friendly for real-life deployment and application.

\myparagraph{Early Recognition}

\input{figureText/fig_early_recognition}

Early recognition aims to classify the video when only observing a small portion of the frames. It gives fast response to the input video stream, which is very useful in real-life application. Here we compare the early video recognition performance on UCF101 dataset. The results are presented in Figure~\ref{fig:early_recognition}. Compared to different ECO models, TSM can give much higher accuracy, especially when only observing a small portion of the frames. For example, when only observing the first 10\% of video frames, TSM can achieve 90\% accuracy, which is 6.6\% higher than the best ECO model and practical for real-life application.





\subsection{Improving Online Video Detection with TSM}
Video understanding from online video streams is very important in real-life scenarios. In this section, we show that we can modify our TSM to achieve online video recognition while with multi-level temporal fusion.

Video detection for online video can be applied to a wide range of robotics, self-driving, etc. But usually 

\input{figureText/tab_compare_online_methods.tex}

==> text/setup.tex <==
\section{Setups}

We first discuss the setup of experiments in this paper.
\myparagraph{Training\&Testing.}
% To evaluate the effectiveness of the proposed method, we conducted experiments on several action recognition datasets. 
To evaluate the effectiveness of the proposed method, we conducted experiments on both action recognition and video object detection.
For action recognition,
% Since many of the action recognition datasets are not large enough and are prone to over-fitting~\cite{wang2016temporal}, 
we followed the common practice~\cite{wang2017non, zolfaghari2018eco, carreira2017quo, xie2018rethinking} to first pre-trained the models on Kinetics~\cite{kay2017kinetics} and then fine-tuned the model to other target datasets like Something-Something~\cite{goyal2017something}, UCF101~\cite{soomro2012ucf101}, and HMDB51~\cite{kuehne2011hmdb}. The fine-tuning is conducted for 25 epochs with initial learning rate 0.001 and decayed by a factor of 0.1 every 10 epochs. We followed the practice in~\cite{wang2016temporal} to fix all the Batch Normalization~\cite{ioffe2015batch} layers except for the first one.
For most of the experiments, we followed the commonly used setting in~\cite{wang2017non} for training and testing. When comparing with previous state-of-the-art efficient models~\cite{zolfaghari2018eco} in Table~\ref{tab:compare_something}, we use the setting in~\cite{zolfaghari2018eco} that uses the same number of frames for both training and testing to make a direct comparison.
For video detection, we followed the same training and testing setting in~\cite{zhu17fgfa, dai16rfcn}, for both the 2D single-frame baseline and our TSM model. The only difference is the TSM inserted into the backbone.
% We used 8 or 16 sampled frames per video for both training and testing.
% We applied similar data augmentation strategy as~\cite{wang2016temporal} for pre-processing: first resizing the raw images such that the shorter side is 256 and then employing a fixed corner+center cropping and scale-jittering. The images are then resized to $224\times 224$ before being fed to the network. 
% Unless otherwise specified, for all the training in our experiments, we used weight decay of 5e-4 and mini-batch SGD optimizer with momentum 0.9. 


\myparagraph{Model.} 
% The performance and efficiency of the overall framework largely relies on the backbone 2D CNN models, which is beyond the contribution of our paper. 
To have an apple-to-apple comparison with the state-of-the-art method~\cite{wang2018videos}, we used the same backbone (ResNet-50) on the same dataset ( Something-Something-V1~\cite{goyal2017something}).This dataset focuses on temporal modeling.  The difference is that \cite{wang2018videos} used 3D ResNet-50, while we used 2D ResNet-50 as the backbone to demonstrate efficiency.
% Another reason is that we need a backbone with residual connection to implement residual version of \method module.

% We discussed several variants of our \netFull model in Section~\ref{sec:appr_variant}. In our experiments, we used the best setting found by our ablation study (Section~\ref{sec:exp_ablation}):  residual temporal shift module with zero padding. We inserted such shift module into each residual unit of the backbone network. A quarter of the channels are shifted.
% ($1/8$ for each direction).


\myparagraph{Datasets.}
Kinetics dataset~\cite{kay2017kinetics} is a large-scale action recognition dataset with 400 classes. As pointed in~\cite{zhou2017temporal, xie2018rethinking}, datasets like Something-Something (V1\&V2)~\cite{goyal2017something}, Charades~\cite{sigurdsson2016hollywood}, and Jester~\cite{jester}  are more focused on modeling the temporal relationships, while UCF101~\cite{soomro2012ucf101}, HMDB51~\cite{kuehne2011hmdb}, and Kinetics~\cite{kay2017kinetics} are less sensitive to temporal relationships. Since our proposed method is a zero-cost approach to conduct temporal modeling, we mainly focus on the dataset with stronger temporal relationships like Something-Something (see Figure~\ref{fig:array_of_time}). Nevertheless, we also observed strong results on the other datasets and reported it.

For video object detection, we conducted experiments on 

\input{figureText/fig_arrow_of_time}
